Dispersion of Mobile Robots: A Study of Memory-Time Trade-offs

We introduce a new problem in the domain of mobile robots, which we term dispersion. In this problem, $n$ robots are placed in an $n$ node graph arbitrarily and must coordinate with each other to reach a final configuration such that exactly one robot is at each node. We study this problem through the lenses of minimizing the memory required by each robot and of minimizing the number of rounds required to achieve dispersion. Dispersion is of interest due to its relationship to the problems of scattering on a graph, exploration using mobile robots, and load balancing on a graph. Additionally, dispersion has an immediate real world application due to its relationship to the problem of recharging electric cars, as each car can be considered a robot and recharging stations and the roads connecting them nodes and edges of a graph respectively. Since recharging is a costly affair relative to traveling, we want to distribute these cars amongst the various available recharge points where communication should be limited to car-to-car interactions. We provide lower bounds on both the memory required for robots to achieve dispersion and the minimum running time to achieve dispersion on any type of graph. We then analyze the trade-offs between time and memory for various types of graphs. We provide time optimal and memory optimal algorithms for several types of graphs and show the power of a little memory in terms of running time.

==> delta-logn-memory.tex <==
% !TEX root = Deterministic-Dispersion-Static.tex
 %please leave the above line untouched. Thanks, Billy.

We look at dispersion on a rooted tree when the memory of each robot is $O(\log n)$ bits.

\subsection{Dispersion on a Rooted Tree}\label{subsec:rooted-tree-logn}
A rooted tree is a tree where all robots start at one node called the root. We look at dispersion on a rooted tree and show that when the memory of each robot is $O(\log n)$ bits, we can achieve dispersion in $O(D^2)$ rounds. Note that a previous version of this paper required robots to have $O(\Delta + \log n)$ bits of memory to achieve the same result. The improvement comes because we convert the variable $fully\_dispersed\_port$ from an array with $\Delta$ bits to a counter using $\log n$ bits. Its purpose remains the same, namely that of checking whether ports of children of the node lead to dispersed subtrees. However, rather than remembering which ports lead to fully dispersed children it just keeps a count of how many.

We define a \textit{fully dispersed subtree rooted at a node} to be a subtree with that node as the root where every node has a robot assigned to it. We use the term \textit{settled} robot to denote a robot which is assigned to a node.

Our algorithm works in stages. Each stage corresponds to (i) the unassigned robots located at the root exploring the tree one level deeper than the previous stage and assigning themselves to empty nodes when possible, and (ii) settled robots updating their information about which ports lead to fully dispersed subtrees. Once a settled robot decides that the subtree rooted at the node it's been assigned to has been fully dispersed, it stops executing the algorithm. 

Each robot is in one of four states: (i) \textit{root}, (ii) \textit{explore}, (iii) \textit{wait}, or (iv) \textit{settled}. Only one robot will be in state $root$ and this is the robot that has been assigned to the root of the tree. This robot executes the algorithm until the subtree rooted at its node is fully dispersed.

A robot in the $settled$ state is essentially assigned to a given node. It maintains a pointer to the port it used to reach this node initially. It also maintains up to $\Delta$ bits of memory, one bit per port, to denote whether a given port has been completely dispersed. We say that a \textit{port has been completely dispersed} when the subtree rooted at the node attached to the port has been fully dispersed. For the remainder of this section, we use level and depth to mean the same thing.

For a given node, define an \textit{unassigned leaf} of the node as a descendant $v$ of the node in the tree such that (i) $v$ is unassigned and (ii) $v$'s immediate parent is assigned a robot. If the given node is itself unassigned a robot but its parent is assigned a robot, we define the number of unassigned leaves of the node as $1$. If the given node and its parent are both unassigned robots, we define its number of unassigned leaves as $0$.

The algorithm uses nine variables, $port\_entered$, $parent\_ptr$, $state$, $dist\_from\_root$, $fully\_dispersed\_port$, $fully\_dispersed$, $num\_robots\_reqd$, $lvl\_cntr$, and $rnd\_cntr$. $port\_entered$ denotes the port through which a robot entered the current node. $parent\_ptr$ is used by a settled robot to indicate the port that that robot used to reach the current node. $state$ indicates the current state of the robot: exploring, settled, or backtracking. $dist\_from\_root$ indicates the distance of the current node from the root. $fully\_dispersed\_port$ is a counter used by settled robots to count how many of their ports leads to fully dispersed subtrees or not. $fully\_dispersed$ is a boolean variable used by settled robots indicating whether the subtree rooted at the robot's node is fully dispersed or not. $num\_robots\_reqd$ is used by a settled robot to indicate how many robots are currently needed to fill its unassigned leaves. $lvl\_cntr$ is used to denote the current maximum level to which robots will explore the tree. $rnd\_cntr$ is used to denote the current round for a given stage.

Every stage $lvl\_cntr$ consists of $2*lvl\_cntr + 1$ rounds. The first $lvl\_cntr$ rounds are used by robots in state $explore$ to traverse the tree to depth $lvl\_cntr-1$ with the help of procedure \emph{Further-Explore}. \emph{Further-Explore} guarantees the following property: in the given stage, if a given node has $x$ unassigned leaves, exactly $x$ robots will be sent to the node in the course of the exploration. This is achieved as follows through \emph{Further-Explore}. For a given node $v$ with children that are settled, in the round where robots reach $v$, the robots assigned to $v$'s children would have moved up to $v$ as well and transmitted the number of unassigned leaves (i.e. number of robots required to be sent through each port). In the subsequent round, these children of $v$ return to their assigned nodes and the robots in state $explore$ know exactly which port to traverse. Once robots reach the parent of an unassigned node, one robot goes to each unassigned node and gets assigned to that node using procedure \emph{Robot-Assignment}.

A robot in $explore$ state not sent from the root changes its state to $wait$ and waits for the beginning of the next stage. Just before the start of a new stage, all nodes in state $wait$ change their state to $explore$. 

The second $lvl\_cntr$ rounds of a stage are used by robots in state $settled$ to propagate information up to their parents about whether the subtree rooted at the corresponding node is fully dispersed or not. This propagation of information occurs in a bottom up fashion with robots at level $lvl\_cntr - 1$ moving up to inform robots at their parents about this information. Subsequently robots at level $lvl\_cntr -1$ move up and inform their parents and so on.

The last round in the stage is used by robots at depth $1$ to move to the $root$ in preparation for the next stage.

\alglanguage{pseudocode}
\begin{algorithm}
	\caption{Robot-Assignment, a procedure run by each robot $u$}
	\label{prot:Robot-Assignment}
	\begin{algorithmic}[1]
		\State Let $\delta$ be degree of node.
		\If {$state = root$}
			\State $num\_robots\_reqd \gets \delta$.
		\Else
			\State $num\_robots\_reqd \gets \delta - 1$, $parent\_ptr \gets port\_entered$.
		\EndIf
		\State Set entries in $fully\_dispersed\_port$ from index $\delta$ to $\Delta - 1$ to $1$.
		\Statex
	\end{algorithmic}
\end{algorithm}

\alglanguage{pseudocode}
\begin{algorithm}
	\caption{Further-Explore, a procedure run by each robot $u$}
	\label{prot:Further-Explore}
	\begin{algorithmic}[1]
		\State Let $\delta$ be degree of node. Order ports in increasing order of port numbers excluding node's robot's $parent\_ptr$ port and any fully dispersed ports. Every robot on the node knows this same order $p_1, \ldots, p_k$ now.
		\State Coordinate with other robots to calculate $u$'s position in the order of increasing labels of exploring robots.
		\If {Nodes from one level down are present on this node and communicating their $num\_robots\_reqd$ values 
			\phantom . \phantom . }
			\State  Robots are assigned to ports in increasing label order until all port's $num\_robots\_reqd$ requirements \phantom . \phantom . \phantom . are filled. Remaining robots stay unassigned.
		\Else
			\State Robots are assigned to ports in increasing label order such that one robot is assigned per port. \newline \phantom . \phantom . \phantom .  Remaining robots stay unassigned.
		\EndIf

		\If {$u$ was assigned to a given port $p_i$}
			\State $u$ moves through port $p_i$.
			\State Increment $dist\_from\_root$.
		\Else
			\State $state \gets wait$.		
		\EndIf
		
		\Statex
	\end{algorithmic}
\end{algorithm}


%NOTE: For a given stage with lvl\_cntr set to some value, we are exploring up to level (lvl\_cntr - 1)  in that stage. Note that root is at level 0.
\alglanguage{pseudocode}
\begin{algorithm}
	\caption{Rooted-Tree-LogN, run by each robot $u$}
	\label{prot:Rooted-Tree-LogN}
	\begin{algorithmic}[1]
		\State Initialize the following values: $port\_entered \gets 0$, $parent\_ptr \gets \bot$, $state \gets explore$, $dist\_from\_root \gets 0$, $fully\_dispersed\_port \gets 0$, $fully\_dispersed \gets FALSE$, $num\_robots\_reqd \gets 0$, $lvl\_cntr \gets 0$.
		
		\If {$u$ is lowest label robot on node}
			\State $state \gets root$.
			\State \emph{Robot-Assignment}.
		\EndIf
		
		\While {$fully\_dispersed = FALSE$} 
			\State Increment $lvl\_cntr$.
			\For {$rnd\_cntr \gets 1, 2 * lvl\_cntr$ + 1}
				\If {$state = root$}
					\If {A robot enters through a given port and its $fully\_dispersed$ bit $= TRUE$}
						\State Increment $fully\_dispersed\_port$.
						\State If $fully\_dispersed\_port = $ degree of node, set $fully\_dispersed \gets TRUE$.
					\Else
						\State Do nothing this round.
					\EndIf
		
				\ElsIf {$state = explore$}
					\State Set $port\_entered \gets$ port entered through.
					\If {No robot assigned to node}
						\State $state \gets settled$
						\State \emph{Robot-Assignment}.
					\EndIf
					\If {$state \neq settled$}
						\State \emph{Further-Explore}.
					\EndIf
		
				\ElsIf {$state = wait$}
					\State Do nothing for round.
					\If {$rnd\_cntr = 2*lvl\_cntr + 1$}
						\State $state \gets explore$
					\EndIf
		
				\ElsIf {$state = settled$}
					\If {($rnd\_cntr = dist\_from\_root - 1$) OR ($rnd\_cntr = 2*lvl\_cntr - dist\_from\_root$) OR \newline \phantom . \phantom . \phantom .
						\phantom . \phantom . \phantom .
						\phantom . \phantom . \phantom . \phantom .
						 ($dist\_from\_root = 1$ AND $rnd\_cntr = 2*lvl\_cntr + 1$ AND $fully\_dispersed = FALSE$) \newline \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom .}
						\State If $fully\_dispersed\_port = $ degree of node $-1$, set $fully\_dispersed \gets TRUE$.
						\State Move through $parent\_ptr$ port.
					\ElsIf {($rnd\_cntr = dist\_from\_root$) OR ($rnd\_cntr = 2*lvl\_cntr - dist\_from\_root + 1$)}
						\State Set $port\_entered \gets$ port entered through.
						\State Communicate with robot(s) at current node and inform them about $u$'s $fully\_dispersed$,
						\newline \phantom . \phantom .\phantom .  \phantom . \phantom .\phantom . \phantom . \phantom .\phantom . \phantom . \phantom . \phantom .
						 $port\_entered$, and $num\_robots\_reqd$ values.
						\State Move through $port\_entered$ port.
					\Else
						\State If any robots inform $u$ about $fully\_dispersed$, increment $fully\_dispersed\_port$. If robots inform $u$  about their \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . 
						 \newline \phantom . \phantom . \phantom . \phantom .  \phantom . \phantom . \phantom .
						 \phantom . \phantom . \phantom . 
						 $num\_robots\_reqd$ values, update $u$'s $num\_robots\_reqd$ value with the sum of all values 
						 \newline \phantom .  \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . \phantom . 
						 heard.
					\EndIf
				\EndIf
			\EndFor
		\EndWhile
		\Statex
	\end{algorithmic}
\end{algorithm}


\begin{theorem} \label{the:rooted-tree-logn}
Algorithm \emph{Rooted-Tree-LogN} can be run by robots with $O(\Delta + \log n)$ bits of memory to ensure dispersion occurs in $O(D^2)$ rounds on rooted trees.
\end{theorem}

\begin{proof}
We first show that algorithm \emph{Rooted-Tree-LogN} only requires every robot to have $O(\Delta + \log n)$ bits of memory and then we subsequently prove the correctness and running time guarantees of the algorithm. Every robot requires $O(\log \Delta)$ bits of memory for $port\_entered$, $O(\log \Delta)$ bits of memory for $parent\_ptr$, $2$ bits of memory for $state$, $O(\log D)$ bits of memory for $dist\_from\_root$, $O(\log n)$ bits of memory for $fully\_dispersed\_port$, $1$ bit of memory for $fully\_dispersed$, $O(\log D)$ bits for $rnd\_cntr$, $O(\log n)$ bits for $num\_robots\_reqd$, $O(\log D)$ bits of memory for $lvl\_cntr$, and $O(\log n)$ bits of memory to compare labels when deciding which robots will be assigned to a given node. Thus each robot requires $O(\Delta + \log n)$ bits of memory in order to successfully run \emph{Rooted-Tree-LogN}.

We prove the correctness of the algorithm by showing that the following induction hypothesis holds true for all $1 \leq i \leq d+1$.

\begin{lemma}\label{lem:stage-clear}
At the end of stage $i$ of \emph{Rooted-Tree-LogN}, all nodes at depth~$\leq i-1$ have robots assigned to them, for all $1 \leq i \leq d+1$.
\end{lemma}

\begin{proof}
At the end of stage $1$, the only node at depth $0$, the root, has a robot assigned to it. So the base case of the induction holds true.

Let us assume that the induction hypothesis holds true for some stage $i$, i.e. at the end of stage $i$ all nodes at depth~$\leq i-1$ have robots assigned to them. We now must show that at the end of stage $i+1$, all nodes at depth $\leq i$ have robots assigned to them. We show this by showing that for every unassigned leaf of the root at the beginning of stage $i+1$, we send exactly one robot to it by the end of stage $i+1$. This implies that all nodes at depth $i$ at the end of stage $i+1$ will have robots assigned to them. Note that once a node has a robot assigned to it, that robot will never be unassigned from that node, so all nodes at previous depth levels continue to have robots assigned to them.

In a given stage $i$, the first $i$ rounds are used for exploration and the second $i$ rounds are used to update robots assigned to nodes about the number of their assigned leaves. Thus at the end of stage $i$, each robot knows the total number of assigned leaves it has, even if it doesn't know which ports lead to how many unassigned leaves. During the first $i+1$ rounds of stage $i+1$, in every round $r$ the following three types of robots will be present in nodes at depth $r-1$: (i) exploring robots, (ii) robots assigned to nodes at depth $r-1$, and (iii) any robots assigned to children of nodes at depth $r-1$ if those children themselves have unassigned leaves. 

For any node at depth $r-1$ at round $r$, one of two cases may occur. Either its children are all unassigned nodes or they are assigned nodes. In the former case, one robot moves down each port leading to an unassigned node. In the latter case, the robots are able to communicate with each other in round $r$ and coordinate such that the number of robots that move down each port is equivalent to the exact number of unassigned leaves of the node attached to that port.

Thus for a given stage $i+1$, after $i+1$ rounds, all nodes at levels $\leq i$ have robots assigned to them.
\end{proof}

Thus, for a depth $d$ tree, after $d+1$ stages, all nodes will have robots assigned to them. Furthermore, for a given node $v$, if the subtree rooted at that node is fully dispersed by the end of a given stage $i$, then by the end of stage $i$ the robot assigned to $v$ will be present on $v$ and will stop executing the algorithm. Thus at the end of stage $d+1$, all robots stop executing the algorithm and dispersion is achieved.

As for running time, since there are $d+1$ stages and each stage takes $O(d)$ rounds, each robot executes a total of $O(d^2) = O(D^2)$ rounds. Thus the running time of \emph{Rooted-Tree-LogN} is $O(D^2)$ rounds.
\end{proof}
